Geometric Active Exploration in Markov Decision Processes: the Benefit of Abstraction

How can a scientist use a Reinforcement Learning (RL) algorithm to design experiments over a dynamical system's state space? In the case of finite and Markovian systems, an area called Active Exploration (AE) relaxes the optimization problem of experiments design into Convex RL, a generalization of RL admitting a wider notion of reward. Unfortunately, this framework is currently not scalable and the potential of AE is hindered by the vastness of experiment spaces typical of scientific discovery applications. However, these spaces are often endowed with natural geometries, e.g., permutation invariance in molecular design, that an agent could leverage to improve the statistical and computational efficiency of AE. To achieve this, we bridge AE and MDP homomorphisms, which offer a way to exploit known geometric structures via abstraction. Towards this goal, we make two fundamental contributions: we extend MDP homomorphisms formalism to Convex RL, and we present, to the best of our knowledge, the first analysis that formally captures the benefit of abstraction via homomorphisms on sample efficiency. Ultimately, we propose the Geometric Active Exploration (GAE) algorithm, which we analyse theoretically and experimentally in environments motivated by problems in scientific discovery.

==> sections/algorithm_old.tex <==
In this section we propose \AlgNameDef, an algorithm that gradually solves the introduced learning problem leveraging the abstract MDP $\overline{\mathcal{M}}_f$. Intuitively, one would like to solve the estimation problem directly in the abstract MDP as the quantity of interest only varies across equivalence classes. However, the quantity of interest is inherently defined as a function of the original state-space and to estimate it, interaction with the original MDP $\mathcal{M}_f$ is necessary. Loosely speaking, the abstract MDP does not exist in the real world and therefore the agent cannot interact with it. Although, performing estimation in the abstract MDP directly is not possible, we show that by leveraging the invariances one can still achieve better sample complexity.

%classes and the abstract state-action space has smaller cardinality leading to better mixing times
\AlgNameLong, presented in Algorithm \ref{alg:GAE}, is based on the algorithmic scheme of Frank-Wolfe for active MDP Exploration (FW-AME) introduced by \cite{tarbouriech2019active}. \AlgNameShort alternates between solving a linear optimization problem and updating the candidate solution via density estimation. The linear optimization problem corresponds to solving a linear MDP where the reward obtained in a certain state-action pair is indicative of the estimation error in said state. In this way, the optimal policy of this MDP tends to visit states where the estimation error is still high more frequently. More explicitly, in the linear optimization problem we solve for a state-action density minimizing the inner product with an optimistic gradient estimate of the objective function. Using the same variance bound as in \cite{tarbouriech2019active}, given in \ref{variance upper bound} the optimistic gradient is given by,
\begin{equation*}
    \nabla \widehat{\overline{\mathcal{L}}}^+_{t_k - 1}(\lambda)[s,a] = \frac{-\sqrt{2 \hat{\sigma}_{t_k - 1}^2(\overline{s}) + \alpha(t_k -1, \overline{s}, \delta)}}{ 2\Phi S \big(\sum_{b \in \mathcal{A}} \sum_{s \in [s]} (\lambda(s, b) + \eta) \big)^{\frac{3}{2}}}.
\end{equation*}

Due to the fact that we marginalize the state-action frequencies over the actions and states in the same equivalence class, the objective function is purely a function of the abstract state. For this reason, the objective function is also invariant over actions and states in the same equivalence class. Crucially, it's optimistic gradient has those invariances too, allowing us to solve the linear optimization problem over $\overline{\Lambda}_{\underline{\eta}}$ only. This is stated more formally in the following proposition.

\begin{restatable}[Gradient Invariances]{proposition}{gradInv}
\label{proposition:gradient_invariance}
    If the quantity of interest $f$ is invariant over states $s$ and $s'$, then the optimistic gradient of the objective function also has invariances,
    \begin{equation*}
    \nabla_\lambda \widehat{\mathcal{L}}^+_{t_k - 1}(\lambda)_{[s,a]} = \nabla_\lambda \widehat{\mathcal{L}}^+_{t_k - 1}(\lambda)_{[s',a']} \:\:\forall s,s' \in [s], \forall a,a'.
    \end{equation*}
\end{restatable}
\rds{add proof in apx}

\begin{restatable}[Constrained Optimality Equivalence]{proposition}{optEquivalence}
\label{proposition:optimality_equivalence}
    Denoting with $\upsilon^+$ the solution to the linear problem in the original domain over $\Lambda_\underline{\eta}$,
    \begin{equation}
        \upsilon^+ = \argmin_{\lambda \in \Lambda_{\underline{\eta}}}  \langle \nabla \widehat{\mathcal{L}}^+_{t_k - 1}(\lambda), \lambda \rangle,
    \end{equation}
    then there exists $\overline{\underline{\eta}}$, such that,
    \begin{equation}
        \overline{\upsilon}^+ = \argmin_{\lambda \in \overline{\Lambda}_{\overline{\underline{\eta}}}} \langle \nabla \overline{\mathcal{L}}^+_{t_k - 1}(\overline{\lambda}), \overline{\lambda} \rangle,
    \end{equation}
    and the following equality holds:
    \begin{equation}
        \overline{\upsilon}^+(\overline{s}, \overline{a}) = \sum_{s \in [\overline{s}]} \sum_{a \in \phi_s^{-1}(\overline{a})} \upsilon^+(s, a)
    \end{equation}
\end{restatable}
\rds{check sub-proof in slack iPad}

\begin{algorithm}
\caption{\AlgNameDef}\label{alg:GAE}
    \begin{algorithmic}[1]
        \STATE \textbf{Input:} $\overline{\lambda}_1 = 1/\Bar{S} 
        \Bar{A}$, $\underline{\eta}$, $h$, $\mathcal{M}$
        \FOR{$k=1,2,...,K-1$}
        \STATE Solve linear optimization problem in abstract domain:
        \begin{equation*}
            \overline{\upsilon}^+_{k+1} = \arg \min_{\overline{\lambda} \in \overline{\Lambda}_{\underline{\eta}}} \langle \nabla \overline{\mathcal{L}}^+_{t_k -1}(\overline{\lambda}_k), \overline{\lambda} \rangle
        \end{equation*}
        \STATE Compute the abstract policy:
        \begin{equation*}
            \overline{\pi}_{k+1}^+(\overline{a}|\overline{s}) = \displaystyle \frac{\overline{\upsilon}^+_{k+1}(\overline{s},\overline{a})}{\sum_{\overline{a}' \in \overline{\mathcal{A}}}\overline{\upsilon}^+_{k+1}(\overline{s},\overline{a}')}
        \end{equation*}
        \STATE Lift the abstract policy back:
        \begin{equation*}
            \pi^+_{k+1}(a|s) = \displaystyle \frac{\overline{\pi}_{k+1}^+(\overline{a}|\overline{s})}{|\{a \in \phi_s^{-1}(\overline{a})\}|}
        \end{equation*}
        \STATE Deploy agent in $\mathcal{M}_f$ for $\tau_k$ steps, sampling $f$ and estimating $\Tilde{\upsilon}_{k+1}$
        \begin{equation*}
            \Tilde{\upsilon}_{k+1}(s,a) = \frac{T_{\tau_k}(s,a)}{\tau_k}
        \end{equation*}
        \STATE Update $\hat{\mu}_{t_{k+1}-1}(\overline{s})$ and $\hat{\sigma}_{t_{k+1}-1}(\overline{s})$ aggregating over equivalence class\\
        \nl{Could put online update but seems a bit ugly}
        \STATE Compute $\Tilde{\overline{\upsilon}}_{k+1}$ aggregating over equivalence classes
        \begin{equation*}
            \Tilde{\overline{\upsilon}}_{k+1}(\overline{s},a) = \sum_{s \in [\overline{s}]} \Tilde{\upsilon}_{k+1}(s,a)
        \end{equation*}
        \nl{Supposedly also some transform on $a$}
        \STATE Update the abstract state-action frequency $\overline{\lambda}_{k+1}$
        \begin{equation*}
            \overline{\lambda}_{k+1} = \frac{\tau_k}{t_{k+1} - 1} \Tilde{\overline{\upsilon}}_{k+1} + \frac{t_k - 1}{t_{k+1} - 1} \overline{\lambda}_{k}
        \end{equation*}
        \ENDFOR
        \STATE \textbf{Return: } $\hat{\mu}_{t_K - 1}$
    \end{algorithmic}
\end{algorithm}
\rds{add explanation of alg almost line by line}

By solving the linear MDP, we obtain an abstract state-action distribution $\overline{\upsilon}^+_{k+1}$ from which the abstract policy $\overline{\pi}^+_{k+1}$ can be computed. As this abstract policy can't be executed directly one needs to \textit{lift} it back to the original domain. Lifting preserves optimality and we follow the same lifting strategy as \cite{derPol2020homomorphic}, where the probability mass is distributed uniformly over the preimage. Subsequently, the agent is deployed in the original MDP following policy $\pi^+_{k+1}$ for $\tau_k$ steps where in every step, the agent conducts an experiment and subsequently, the observations are aggregated over different equivalence classes to update the sample mean and standard deviations, $\hat{\mu}_{t_{k+1}-1}$ and $\hat{\mu}_{t_{k+1}-1}$. Concurrently, the empirical density $\tilde{\upsilon}_{k+1}$ is estimated form the $\tau_k$ steps and then aggregated to obtain it's abstract version $\tilde{\overline{\upsilon}}_{k+1}$. Ultimately, the candidate solution $\overline{\lambda}_k$ is updated using the same update rule as in \cite{tarbouriech2019active}.






%Due to the invariances in the quantity of interest, the gradient of the objective function also exhibits invariances, which allows us to solve the linear optimization problem over the abstract state-action distributions.


%in general I'd put some extra lines and focus on the steps that differ from FW-AME (eg. input h, abstract MDP computation if needed, resolution in abstract MDP, line for computation of abstract empirical  density once original density is computed) + add return of estimate of f as we give guarantees for it?



%We consider the setting in which the variance of the quantity of interest $f$ is unknown a priori and heteroscedastic over different equivalence classes. Furthermore, we assume that the dynamics $P$ of the original MDP $\mathcal{M}_f$ are known. \nl{Add intuition for how one could relax this assumption.}



%However, since we want to solve an estimation problem on a quantity defined over the original state space, one must necessarily interact with the original system. 

%and is perhaps of simpler structure.

%However, interacting with the abstract MDP implies transitioning between abstract states according to the transition model $\overline{P}$, which is generally different from the original $P$. Interacting with the abstract MDP is therefore not possible as the dynamics of the underlying system cannot be changed. Although, direct interaction with the abstract MDP is not possible, we show in the following the one can still leverage it to be more sample efficient.

%\AlgNameLong extends Frank-Wolfe for Active MDP Exploration (FW-AME) algorithm introduced by \cite{tarbouriech2019active}. FW-AME is based on the general Frank-Wolfe scheme \cite{pmlr-v28-jaggi13} where one alternates between solving a linear optimization problem and gradually updating the candidate solution. \nl{Here potentially elaborate on why the solution to the linear problem cannot be executed directly as explained in tarbouriech and potentially elaborate on the general convex RL scheme.}


%- present algorithmic scheme very high level (typical convex RL scheme)

%- pseudocode algorithm with 'line-by-line' explanation

%- present main algorithm intuitions: (1) proposition, f state invariances induce state-action r invariances (2) solve abstract LPs/linear MDPs rather than original ones, (3) density estimation aggregates hence concentrates faster even though policy is released in original CMP.

%The core idea of our approach is to exploit the symmetries in the environment to estimate our unknown function faster. In this work, we assume the symmetries to be known a priori, i.e. they do not have to be learned via exploration. In particular, we assume that the agent has access to the homomorphism function $\upsilon$ and the transition kernel $P$ at the beginning of the task. Then, the agent will exploit this to compute and construct the abstract MDP $\mathcal{\overline{\cmp_f}}$. As we mentioned previously, the goal of the agent is to optimize the asymptotic relaxation of the proxy objective $\mathcal{L}_{\infty}^{\eupsilonlon}=\frac{1}{S}\sum_{s \in S} \frac{\sqrt{2 \hat{\sigma}^2_{\pi, n}(s)}}{\sqrt{\sum_{b \in \mathcal{A}} \lambda(s, b)}}$. However, since we want to exploit the abstract MDP and the symmetries of the environment, we want the agent to solve the optimization problem in the abstract MDP directly, as this will result in a faster method. In order to do so, we would like the agent to act in the abstract MDP directly instead of the actual environment. \fa{add proposition about invariances induced by f and the gradients, have to see exactly where to put it}. This is not possible in practice though, where the agent, even if it plans to act in the abstract environment, always lies in a state of the real environment and once it takes an action, this will correspond to a movement to a new state of the real environment. Here it might seem that our method breaks, as our aim would be to act in the abstract MDP only. However, there is a key insight which follows from the stability assumption that allows us the agent to plan in the abstract MDP while not paying attention to which exact state of the real environment it will end up: in particular, stability ensures that when the agent occupies a state of a given equivalence class, then once it takes an action it will have the same probability of ending up in the equivalence class of the next state as if he was in any other state of the current equivalent class (given it takes the same action). \fa{maybe a simple picture could be of help here to give better intuition to the readers}. Hence, even if the agent is actually moving in the real environment, stability implies that this is essentially equivalent to acting in the abstract MDP if the agent plans to act optimally there. \fa{rewrite last sentence better}. 
%\\
%Since we want the agent to solve the task in the abstract MDP, the agent will actually minimize the abstract version of the aforementioned aymptotic relaxation, namely $\overline{\mathcal{L}}_{\infty}^{\eupsilonlon}=\frac{1}{\Phi S}\sum_{\overline{s} \in \overline{S}} \frac{\sqrt{2 \hat{\sigma}^2_{\pi, n}(\overline{s})}}{\sqrt{\sum_{b \in \mathcal{A}} \overline{\lambda}(\overline{s}, b)}}$. We note that this is a convex function in the state-occupancy measure $\overline{\lambda}$ and hence the optimization problem can be solved using techniques coming from the Convex RL literature \fa{add references}. 
%\\
%In particular, here we adopt a Frank-Wolfe like strategy, where at each iteration the agent has to solve a Linear Program in $\overline{\lambda}$ which is equivalent to a classical RL instance where the reward function is equivalent to the estimated gradient (since the true variance is unknown) of the objective function $\overline{\mathcal{L}}_{\infty}^{\eupsilonlon}$. From this, the agent computes the policy corresponding to the optimal solution of the RL instance mentioned above. Now comes the second delicate step of the algorithm: the policy we have just calculated is an abstract policy $\overline{\pi}(\overline{a}|\overline{s})$ that is optimal and can be deployed in the abstract MDP. However, we would be interested in a lifted policy that can be deployed in the real environment since, as we mentioned above, the agent is constricted to act in the real world even if he "imagines" to act in the abstract environment. Then the following question arise: how should we "lift" the abstract policy back? Does lifting preserve optimality (i.e. is it optimal for the RL instance with the gradient of the original objective function)? Astonishingly, one can prove that the invariances in the action space are such that the lifted policy is exactly the same as the abstract one, which leads us to the following proposition: \fa{add Proposition that lifted policy is the same as abstract one}. This is nice since this translates into the fact that in practice we do not have to do any computational effort to calculate the lifted policy, which was not obvious a priori. In addition, the lifted policy also preserves optimality as desired, as we prove in the following: \fa{add Proposition that lifted policy is optimal wrt gradient of original objective}. This is crucial, since it means that at every step of Frank-Wolfe we preserve optimality. Since this happens at each step of the algorithm, this translates into the fact that our strategy is optimal overall \fa{do we maybe want to be a bit more formal here?}.
%\\
%Once we have calculated the lifted policy, we can release the agent deploying this policy in the environment and we will estimate the corresponding state-action occupancy measure. We will then use this to update the mixture of state-action frequencies, which in turn is used to evaluate the gradient of the objective at next time step. Once we have repeated this step a sufficiently large amount of times, we will return our final estimate for the unknown function $f$. Note that differently from usual Frank-Wolfe or Convex-RL schemes, here we do not have to return the final mixture policy, as our main goal is to estimate the unknown quantity.
%\fa{write Pseudo Code}
%\fa{in the algorithm, we haven't specified where we collect the samples to estimate the function}



%%%%%%%%%%% Commented out Noah's rewriting

%We consider the setting, where the variance $\sigma^2$ of the quantity of interest $f$ is unknown a priori and heteroscedastic over different equivalence classes but constant within an equivalence class.


%To leverage the abstract CMP, we make the following simplifying assumptions.


%\begin{restatable} [] {assumption}{knownInvariances}
%The homomorphism $h: (\upsilon, \{\phi_s | s \in \mathcal{S}\})$ mapping the MDP $\mathcal{M}_f$ to it's abstract version $\overline{\mathcal{M}_f}$ is known.
%\end{restatable}
%\begin{restatable} [] {assumption}{knownTransitions}
%The transition model $P$ is known.
%\end{restatable}

==> sections/conditions_abstraction.tex <==
Until this point, we have assumed to have access to a known MDP homomorphism $h = (\psi, \{\phi_s \mid s \in \Sspace\})$. In this section, we discuss how $h$ can be built in practice in two major ways: either (i) encoding known geometric inductive biases on $f$ and $P$ as previously discussed, or (ii) leveraging model-minimization algorithms to discover symmetries or to learn a MDP homomorphism automatically. 

\mypar{Abstraction via Geometric Inductive Biases}~~
If the dynamics $P$ is known to satisfy a superset of the symmetries satisfied by $f$, then we have an \emph{MDP with symmetries}. Luckily, due to the roto-translation invariance of $P$ this is the case in a vast variety of estimation processes in real-world systems~\cite{derPol2020homomorphic}. For instance, in the illustrative example in Fig. \ref{fig:diffusion_drawing}, both the dynamics $P$ and the reward function $r$ satisfy radial symmetries centered in the source of the diffusion process. 

In this case, there exists a set of transformations on the state-action space to which the reward $r: \Sspace \times \Aspace \xrightarrow[]{} \mathbb{R}$ and the dynamics $P$ are invariant. We define a \emph{state transformation} $L_g: \Sspace \to \Sspace$ and a \emph{state-dependent action transformation} $K^s_g: \Aspace \to \Aspace$, and express the invariances of $r$ and $P$ as
\begin{align}
    r(s,a) &= r(L_g[s], K^s_g[a]) \label{eq:mdp_sym_r}\\
    P(s' \mid s,a) &= P(L_g[s'] \mid L_g[s], K^s_g[a]) \label{eq:mdp_sym_P}
\end{align}
for all $g \in G, s \in \Sspace, a \in \Aspace$.

Given an MDP with symmetries $\cmp_r$, it is possible to define a \emph{group-structured} abstract MDP $\overline{\cmp_r}$, by mapping $(s,a)$ and each state-action pair obtained by applying transformations $L_g$ and $K_g$, to the same abstract state-action pair $(\sAbs, \aAbs) \coloneqq (\psi(s), \phi_s(a))$, namely we have that:
\begin{equation*}
    (\psi(s), \phi_s(a)) = (\psi(L_g[s]), \phi_{L_g[s]}(K_g^s[a]))
\end{equation*}
for all $g \in G, s \in \Sspace, a \in \Aspace$. This abstraction process is depicted in Fig. \ref{fig:diffusion_drawing}. Notice that, in practice, computing the abstract MDP $\overline{\cmp_r}$ induced by a set of symmetries is efficient since it requires to perform one sweep over $\Sspace \times \Aspace$.

% In the case of the diffusion process in Fig. \ref{fig:diffusion_drawing}, given the action set $\Aspace = \{$inward, outward, clockwise, anti-clockwise, stay$\}$ for a fixed action $a \in \Aspace$, each state-action $(s,a)$ with state $s$ equally distant from the center will be mapped to a unique abstract state-action pair $(\sAbs, \aAbs) \in \SspaceAbs \times \AspaceAbs$. Therefore, $\SspaceAbs$ can be imagined as a discrete line where each $s \in \SspaceAbs$ represents the equivalence class of all states equally distanced from the source point. If we consider an instance with a total of $S=100$ states distributed across $20$ rays, the abstract MDP induced by the radial symmetries will have $\overline{S}=5$ abstract states.

\mypar{Abstraction via Automatic Model Minimization}~~
\looseness -1 While in certain applications \eg molecular design or environmental sensing, geometric priors on $f$ and $P$ are known, for a arguably wider set of applications geometric structure is not known or it is not human-interpretable. In these cases, one can leverage algorithms that automatically discover symmetries in the environment~\cite{angelotti2021expert, narayanamurthy2008hardness} or directly learn a MDP homomorphism~\cite{mavor2022simple, biza2018online, wolfe2006decision, pmlr-v162-mondal22a}. 
% Notice that while promising and relevant, the problems of symmetry discovery and MDP homomorphism learning are orthogonal to the contributions presented in this work.

==> tikzimages/fullmdp.tex <==
\begin{tikzpicture}[>=Stealth, node distance=2cm, state/.style = {draw, circle}]
    \def\N{6} % Number of states
    \def\NumCircles{3} % Number of circles
    \def\RadiusStep{0.7} % Step increase in radius for each circle

    % Define colors for different circles
    \def\Colors{{"blue!30", "red!30", "red!30", "yellow!30", "blue!30", "red!30", "red!30", "yellow!30"}}

    % Create states in circles
    \foreach \circle in {1,...,\NumCircles} {
        \pgfmathsetmacro\CurrentRadius{\RadiusStep * \circle}
        \pgfmathsetmacro\Color{\Colors[\circle-1]}
        \foreach \s in {1,...,\N} {
            \node[state, fill=\Color] (circle\circle-\s) at ({360/\N * (\s - 1)}:\CurrentRadius cm) {};
        }
    }

    % Connect states within each circle
    \foreach \circle in {1,...,\NumCircles} {
        \foreach \s in {1,...,\N} {
            \pgfmathtruncatemacro{\nexts}{mod(\s,\N)+1}
            \draw[<->,bend right] (circle\circle-\s) to (circle\circle-\nexts);
        }
    }

    \foreach \circle in {2,...,\NumCircles} {
        \pgfmathsetmacro\nextcircle{int(\circle -1)}
        \foreach \s in {1,...,\N} {
            \draw[<->] (circle\circle-\s) -- (circle\nextcircle-\s);
        }
    }
\end{tikzpicture}

==> tikzimages/hom1.tex <==
\begin{tikzpicture}[>=Stealth, node distance=2cm, state/.style = {draw, circle}]
    \def\N{6} % Number of states
    \def\NumCircles{2} % Number of circles
    \def\RadiusStep{0.7} % Step increase in radius for each circle

    % Define colors for different circles
    \def\Colors{{"blue!30", "red!30", "red!30", "yellow!30", "blue!30", "red!30", "red!30", "yellow!30"}}

    % Create states in circles
    \foreach \circle in {1,...,\NumCircles} {
        \pgfmathsetmacro\CurrentRadius{\RadiusStep * \circle}
        \pgfmathsetmacro\Color{\Colors[\circle-1]}
        \foreach \s in {1,...,\N} {
            \node[state, fill=\Color] (circle\circle-\s) at ({360/\N * (\s - 1)}:\CurrentRadius cm) {};
        }
    }

    % Connect states within each circle
    \foreach \circle in {1,...,\NumCircles} {
        \foreach \s in {1,...,\N} {
            \pgfmathtruncatemacro{\nexts}{mod(\s,\N)+1}
            \draw[<->,bend right] (circle\circle-\s) to (circle\circle-\nexts);
        }
    }

    \foreach \circle in {2,...,\NumCircles} {
        \pgfmathsetmacro\nextcircle{int(\circle -1)}
        \foreach \s in {1,...,\N} {
            \draw[<->] (circle\circle-\s) -- (circle\nextcircle-\s);
        }
    }
\end{tikzpicture}

==> tikzimages/hom2.tex <==
\begin{tikzpicture}[>=Stealth, node distance=2cm, state/.style = {draw, circle}]
    \def\N{3} % Number of states
    \def\NumCircles{2} % Number of circles
    \def\RadiusStep{0.7} % Step increase in radius for each circle

    % Define colors for different circles
    \def\Colors{{"blue!30", "red!30", "red!30", "yellow!30", "blue!30", "red!30", "red!30", "yellow!30"}}

    % Create states in circles
    \foreach \circle in {1,...,\NumCircles} {
        \pgfmathsetmacro\CurrentRadius{\RadiusStep * \circle}
        \pgfmathsetmacro\Color{\Colors[\circle-1]}
        \foreach \s in {1,...,\N} {
            \node[state, fill=\Color] (circle\circle-\s) at ({360/\N * (\s - 1)}:\CurrentRadius cm) {};
        }
    }

    % Connect states within each circle
    \foreach \circle in {1,...,\NumCircles} {
        \foreach \s in {1,...,\N} {
            \pgfmathtruncatemacro{\nexts}{mod(\s,\N)+1}
            \draw[<->,bend right] (circle\circle-\s) to (circle\circle-\nexts);
        }
    }

    \foreach \circle in {2,...,\NumCircles} {
        \pgfmathsetmacro\nextcircle{int(\circle -1)}
        \foreach \s in {1,...,\N} {
            \draw[<->] (circle\circle-\s) -- (circle\nextcircle-\s);
        }
    }
\end{tikzpicture}

==> tikzimages/hom3.tex <==
\begin{tikzpicture}[>=Stealth, node distance=2cm, state/.style = {draw, circle}]
    \def\N{1} % Number of states
    \def\NumCircles{2} % Number of circles
    \def\RadiusStep{1} % Step increase in radius for each circle

    % Define colors for different circles
    \def\Colors{{"blue!30", "red!30", "red!30", "yellow!30", "blue!30", "red!30", "red!30", "yellow!30"}}

    % Create states in circles
    \foreach \circle in {1,...,\NumCircles} {
        \pgfmathsetmacro\CurrentRadius{\RadiusStep * \circle}
        \pgfmathsetmacro\Color{\Colors[\circle-1]}
        \foreach \s in {1,...,\N} {
            \node[state, fill=\Color] (circle\circle-\s) at ({360/\N * (\s - 1)}:\CurrentRadius cm) {};
        }
    }

    \foreach \circle in {2,...,\NumCircles} {
        \pgfmathsetmacro\nextcircle{int(\circle -1)}
        \foreach \s in {1,...,\N} {
            \draw[<->] (circle\circle-\s) -- (circle\nextcircle-\s);
        }
    }
\end{tikzpicture}
